Multi-LogiEval: Towards Evaluating Multi-Step Logical Reasoning Ability of Large Language Models

As Large Language Models (LLMs) continue to exhibit remarkable performance in natural language understanding tasks, there is a crucial need to measure their ability for human-like multi-step logical reasoning. Existing logical reasoning evaluation benchmarks often focus primarily on simplistic single-step or multi-step reasoning with a limited set of inference rules. Furthermore, the lack of datasets for evaluating non-monotonic reasoning represents a crucial gap since it aligns more closely with human-like reasoning. To address these limitations, we propose Multi-LogiEval, a comprehensive evaluation dataset encompassing multi-step logical reasoning with various inference rules and depths. Multi-LogiEval covers three logic types--propositional, first-order, and non-monotonic--consisting of more than 30 inference rules and more than 60 of their combinations with various depths. Leveraging this dataset, we conduct evaluations on a range of LLMs including GPT-4, ChatGPT, Gemini-Pro, Yi, Orca, and Mistral, employing a zero-shot chain-of-thought. Experimental results show that there is a significant drop in the performance of LLMs as the reasoning steps/depth increases (average accuracy of ~68% at depth-1 to ~43% at depth-5). We further conduct a thorough investigation of reasoning chains generated by LLMs which reveals several important findings. We believe that Multi-LogiEval facilitates future research for evaluating and enhancing the logical reasoning ability of LLMs. Data is available at https://github.com/Mihir3009/Multi-LogiEval.

==> tables/NM_2_example.tex <==
% \begin{table}[]
% \begin{tabular}{clcc}
% \textbf{Rules}                                                               & \multicolumn{1}{c}{\textbf{Combination}}                                                                                                   & \textbf{Context} & \textbf{Question} \\
% \begin{tabular}[c]{@{}c@{}}BDR\_DRD\_DS\\   (1)     (2)     (3)\end{tabular} & \begin{tabular}[c]{@{}l@{}}X: Conclusion of BDR (1)\\ Y: Conclusion of DRD (2)\\ \\ X, Y follows DS (3):\\ ((X ∨ Y) ∧ ¬X) ⊢ Y\end{tabular} & (X ∨ Y) ∧ ¬X)    & Y                
% \end{tabular}
% \end{table}


% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[htbp]
  \centering
    \begin{tabular}{p{7.5em}|p{12em}|p{7em}|p{4em}}
    \toprule
    \textbf{Rules} & \textbf{Combination} & \textbf{Context} & \textbf{Question} \\
    \midrule \midrule
    
    $BDR\_DRD\_DS$ \newline{} $(1)\_(2)\_(3)$ & 
    X: Conclusion of BDR (1)\newline{}Y: Conclusion of DRD (2)\newline{}\newline{} X, Y follows DS (3):\newline{}$((X \vee Y) \wedge \neg X)$ $\vdash$ Y 
    & BDR, DRD, and $(X \vee Y) \wedge \neg X)$ 
    & Y \\ \midrule

    
    \bottomrule
    \end{tabular}%
    \caption{Add caption}
  \label{tab:addlabel}%
\end{table*}%


==> tables/fewshot_comparision_gpt3.5.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c}
\toprule
\multirow{2}{*}{\textbf{n-shot}} & \multicolumn{5}{c|}{\textbf{Propositional}} & \multicolumn{5}{c|}{\textbf{First-Order}} & \multicolumn{2}{c}{\textbf{Non-Monotonic}}
                                \\ \cmidrule{2-13} 
                                 & \multicolumn{1}{c|}{\textbf{$d_1$}} & \multicolumn{1}{c|}{\textbf{$d_2$}} & \multicolumn{1}{c|}{\textbf{$d_3$}} & \multicolumn{1}{c|}{\textbf{$d_4$}} & \textbf{$d_5$} & \multicolumn{1}{c|}{\textbf{$d_1$}} & \multicolumn{1}{c|}{\textbf{$d_2$}} & \multicolumn{1}{c|}{\textbf{$d_3$}} & \multicolumn{1}{c|}{\textbf{$d_4$}} & \textbf{$d_5$} & \multicolumn{1}{c|}{\textbf{$d_1$}} & \textbf{$d_2$} \\ \midrule \midrule

0-shot &76.87\% &44.00\% &41.80\% &27.14\% &28.00\% &78.34\% &72.67\% &47.50\% &30.15\% &16.67\% &25.63\% &27.55\% \\

%87.22\% &	84.72\% &	79.40\% &	71.42\% &	82.66\% &	93.34\% &	91.88\% &	75.50\% &	58.80\% &	44.67\% &	75.00\% &	57.11\% \\
1-shot &86.25\% &	84.72\% &	79.40\% &	71.42\% &	82.66\% &	93.34\% &	91.88\% &	75.50\% &	58.80\% &	44.67\% &	75.00\% &	57.11\% \\

%87.78\% &	88.18\% &	80.60\% &	79.43\% &	88.67\% &	95.56\% &	94.20\% &	82.00\% &	65.97\% &	52.00\% &	78.12\% &	51.77\% \\

2-shot &86.25\% &	88.18\% &	80.60\% &	79.43\% &	88.67\% &	95.56\% &	94.20\% &	82.00\% &	65.97\% &	52.00\% &	78.12\% &	51.77\% \\

%90.55\% &	89.27\% &	80.40\% &	85.42\% &	92\% &	95.56\% &	97.10\% &	87.50\% &	69.55\% &	57.33\% &	76.87\% &	50.88\% \\

3-shot &89.37\% &	89.27\% &	80.40\% &	85.42\% &	92.00\% &	95.56\% &	97.10\% &	87.50\% &	69.55\% &	57.33\% &	76.87\% &	50.88\% \\

%86.11%	76.54%	70.55%	65.85%	72.83%	90.70%	88.96%	73.13%	56.12%	42.67%	63.91%	46.83%
\midrule
Avg. &84.69\% &	76.54\% &	70.55\% &	65.85\% & 72.83\% &	90.70\% &	88.96\% &	73.13\% &	56.12\% &	42.67\% &	63.91\% &	46.83\% \\

\bottomrule
\end{tabular}
}
\caption{Few shot Evaluation of ChatGPT in terms of accuracy on \textit{Multi-LogiEval}.}
\label{tab:fewshot_gpt3.5}%
\end{table*}



==> tables/validation_question.tex <==
\begin{table*}[htbp]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{m{5cm}|m{5cm}|m{5cm}}
\toprule
\multicolumn{1}{c|}{\textbf{PL}}                                                                            &  \multicolumn{1}{c|}{\textbf{FOL}}                                                                                                    & \multicolumn{1}{c}{\textbf{NM}}                                                                                                                               \\ \midrule\midrule
1. Does the story contain sentences that follow the structure of the mentioned rules?                      & 1. Does the story contain sentences that follow the structure of mentioned rules?                      & 1. Does the story contain all the assumptions from Rule 1 and Rule 2 without directly referencing rules, objects, or properties? \\ \midrule
2. Does the story use real values for the entities (P1, P2, C1, ...)?                                      & 2. Does the story use only indefinite pronouns for the elements corresponding to all rules?            & 2. Are the conclusions (X and Y) logically derived based on the assumptions stated in Rule 1 and Rule 2?                         \\ \midrule
3. Does the story use entity labels (P1, P2, C1, ...) within the narrative?                                & 3. Does the story use any proper noun for the elements corresponding to all rules?                     & 3. Does the story avoid explicitly mentioning rules, objects, or properties from the logical framework?                          \\ \midrule
4. Do the reasoning questions accurately reflect the logical structure of the story and rules?             & 4. Are the sentences in the story logically connected to establish a causal relationship as per Rules? & 4. Do the assumptions in the story logically connect to form the conclusions (X and Y)?                                          \\ \midrule
5. Are the sentences in the story logically connected to establish a causal relationship as per the rules? & 5. Does the story maintain consistency in using indefinite pronouns throughout?                        & 5. Does the story follow the structure of Rule 3 in presenting a situation for proper conclusion?                                \\ \midrule
6. Is the conclusion drawn in the story logically connected as mentioned in the given rules?               & 6. Is the conclusion drawn in the story logically connected as mentioned in the given rules?           & 6. Is the language in the story clear and concise, avoiding unnecessary details that do not contribute to the logical framework? \\ \midrule
7. Do the reasoning questions directly relate to the content of the story and rules?                       & 7. Is the question clear and directly related to the content of the story?                             & 7. Does the question derived from the story follow the structure of Rule 3 and align with the assumptions made in Rule 3?        \\ \midrule
8. Is the language in the story concise and clear, avoiding ambiguity?                                     & 8. Is the language in the story concise and clear, avoiding ambiguity?                                 & 8. Is the question referring to rules, objects, or properties and not generalized?                                               \\ \midrule
9. Do the reasoning questions accurately follow the logical inferences derived from the story and rules?   & 9. Does the question accurately follows the logical inference derived from the story?                  & 9. Does the question accurately follows the logical inference derived from the story based on the assumptions in Rule 3?      \\ \bottomrule   
\end{tabular}
}
\caption{Validation questions used to validate samples for PL, FOL and NM.}
\label{tab:val_questions}
\end{table*}
